CapsNet for Medical Image Segmentation

Convolutional Neural Networks (CNNs) have been successful in solving tasks in computer vision including medical image segmentation due to their ability to automatically extract features from unstructured data. However, CNNs are sensitive to rotation and affine transformation and their success relies on huge-scale labeled datasets capturing various input variations. This network paradigm has posed challenges at scale because acquiring annotated data for medical segmentation is expensive, and strict privacy regulations. Furthermore, visual representation learning with CNNs has its own flaws, e.g., it is arguable that the pooling layer in traditional CNNs tends to discard positional information and CNNs tend to fail on input images that differ in orientations and sizes. Capsule network (CapsNet) is a recent new architecture that has achieved better robustness in representation learning by replacing pooling layers with dynamic routing and convolutional strides, which has shown potential results on popular tasks such as classification, recognition, segmentation, and natural language processing. Different from CNNs, which result in scalar outputs, CapsNet returns vector outputs, which aim to preserve the part-whole relationships. In this work, we first introduce the limitations of CNNs and fundamentals of CapsNet. We then provide recent developments of CapsNet for the task of medical image segmentation. We finally discuss various effective network architectures to implement a CapsNet for both 2D images and 3D volumetric medical image segmentation.

==> aboutauthors.tex <==
\begin{frontmatter}
\chapter*{Biography}
\end{frontmatter}

\begin{biography}

  \section*{Sir Stanley Davidson (1894--1981)}

  One or more blank lines denote the end of a paragraph.  The ends of\index{index}
  words and sentences are marked by spaces. It doesn't matter how many
  spaces you type; one is as good as 100.  The end of a line counts as
  a space.

\end{biography}


==> chapter2.tex <==
\cleardoublepage

\begin{frontmatter}
\chapter{Capsule Networks for Medical Imaging}\label{chap2}
\subchapter{Chapter Subtitle}

\begin{aug}
\author[addressrefs={ad1,ad2}]%
  {\fnm{Firstname}   \snm{Surname}}%
  %{\fnm{Firstname}   \snm{Surname}\footnote{This is author footnote}}%
\author[addressrefs={ad2}]%
 {\fnm{Firstname} \snm{Surname}}%
\address[id=ad1]%
  {Short Address}%
\address[id=ad2]%
  {Long Address}%
\end{aug}


% \minitoc

%
\begin{chapterpoints}%[Chapter Points]
\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
\end{chapterpoints}

\begin{dispquote}

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
  
  \source{Name}

\end{dispquote}

\end{frontmatter}


\section{Capsule Network: Basic}\label{sec2.1}
\section{2D Capsule Network}
\section{3D Capsule Network}
\section{Comparison between CapsNets and CNNs}


==> contributors.tex <==
%% Contributors list %%
\begin{frontmatter}
\chapter*{Contributors}
\end{frontmatter}

\begin{contributorslist}
  \name{Greg N. Gregoriou} is Professor of Finance in the School of
  Business and Economics at State University of New York at
  Plattsburgh. He obtained his Ph.D. (finance) from the University of
  Quebec at Montreal and is hedge-fund editor for the peer-reviewed
  scientific journal Derivatives Use, Trading and Regulation and
  editorial board member for the Journal of Wealth Management, and the
  Journal of Risk and Financial Institutions. He has written more than
  50 articles on hedge funds and managed futures in various U.S. and
  U.K. peer-reviewed publications, including (among others) the
  Journal of Portfolio Management, Journal of Derivatives Accounting,
  Journal of Futures Markets, European Journal of Operational
  Research, Annals of Operations Research, European Journal of
  Finance, and Journal of Asset Management. He has edited 18 books for
  Elsevier, Wiley, Palgrave-MacMillan, and Risk and has coauthored one
  book for Wiley.

  \name{Donald F. Dansereau} Department of Psychology, Texas Christian
  University, Fort worth, Texas

  \name{Ruth Garner} Department of Educational Psychology, Texas A \&
  M University, College Station, Texas
\end{contributorslist}



==> dedication.tex <==
  %% Dedication page
\begin{dedication}
  %% Dedication
  %% can be few\\
  %% lines long
\end{dedication}


==> listoffigures.tex <==
\begin{frontmatter}
\chapter*{List of Figures}
\end{frontmatter}

\listoffigures


==> part.tex <==
\cleardoublepage
\begin{frontmatter}
%\part{}
\end{frontmatter}

% Text ...


==> part1.tex <==
\begin{frontmatter}
\part{Part title}\label{part1}
\end{frontmatter}

% Text ...


==> preface.tex <==
\cleardoublepage
% \begin{frontmatter}
% \chapter*{Preface}%
%\addcontentsline{toc}{schapter}{Preface}
% \end{frontmatter}


%  The ends of words and sentences are marked by spaces. It doesn't
%  matter how many spaces you type; one is as good as 100.  The end of
%  a line counts as a space.

%  The ends of words and sentences are marked by spaces. It doesn't
%  matter how many spaces you type; one is as good as 100.  The end of
%  a line counts as a space.

%  The ends of words and sentences are marked by spaces. It doesn't
%  matter how many spaces you type; one is as good as 100.  The end of
%  a line counts as a space.

% \source%
% {%
%   \author{Name}\\%
  % \address{Location}\\%
  % \date{Month Year}%
% }


==> references.tex <==
%\begin{frontmatter}
%  \chapter*{References}
%  \markboth{References}{References}
%\end{frontmatter}

\begin{thebibliography}{10}

% \bibitem{..}
% \bibitem[]{..}

\end{thebibliography}

==> tableofcontents.tex <==
%% Table of Contents %%
\begin{frontmatter}
\chapter*{Contents}
\end{frontmatter}

\tableofcontents


==> titlepage.tex <==
%% Title Page %%
\begin{titlepage}%
  \begin{titlepagerule}
    % \title{Book title}
    %\subtitle{Book Subtitle}
    %\volume{2}
  \end{titlepagerule}

%   \edition{1st edition}

%  \editedby{Edited by}

%   \author{Author Firstname  Surname}
%   \address{Author Address\\Department of Chemistry\\University of Florida}

%   \author{Author Firstname  Surname}
%   \address{Author Address}
\end{titlepage}

